Cross-Modal Self-Attention Network for Referring Image Segmentation

We consider the problem of referring image segmentation. Given an input image and a natural language expression, the goal is to segment the object referred by the language expression in the image. Existing works in this area treat the language expression and the input image separately in their representations. They do not sufficiently capture long-range correlations between these two modalities. In this paper, we propose a cross-modal self-attention (CMSA) module that effectively captures the long-range dependencies between linguistic and visual features. Our model can adaptively focus on informative words in the referring expression and important regions in the input image. In addition, we propose a gated multi-level fusion module to selectively integrate self-attentive cross-modal features corresponding to different levels in the image. This module controls the information flow of features at different levels. We validate the proposed approach on four evaluation datasets. Our proposed approach consistently outperforms existing state-of-the-art methods.

==> experiment.tex <==
\input tab_miou.tex
\input tab_ab.tex

\section{Experiments}\label{sec:experiment}
In this section, we first introduce the datasets and experimental setup in Sec.~\ref{sec:dataset}. Then we present the main results of our method and compare with other state-of-the-art in Sec.~\ref{sec:result}. Finally, we perform detailed ablation analysis to demonstrate the relative contribution of each component of our proposed method in Sec.~\ref{sec:ab}. We also provide qualitative visualization to help gain insight of our model.

\subsection{Datasets and Setup}\label{sec:dataset}

\noindent{\bf Implementation details}: Following previous work~\cite{liu2017recurrent, li2018referring, shi2018key}, we adopt DeepLab-101~\cite{chen2016deeplab} as our backbone network. We also follow \cite{liu2017recurrent} to keep the maximum length of query expression as $20$, and embed each expression word to a vector of $C_l=1000$ dimensions. Given an input image, we resize it to $320\times320$ and use the outputs of DeepLab-101 ResNet blocks $Res3,Res4,Res5$ as the inputs for multimodal features. The dimension used in $X^{(i)}$ for gated fusion is fixed to $500$.
The network is trained with 
%Adam optimizer~\cite{kingma2014adam} with 
an initial learning rate of $2.5e^{-4}$ and weight decay of $5e^{-4}$. The learning rate is gradually decreased using the polynomial policy with power of $0.9$. For fair comparisons, the final segmentation results are refined by DenseCRF~\cite{krahenbuhl2011efficient}.

\noindent{\bf Datasets}: We perform extensive experiments on four referring image segmentation datasets: UNC~\cite{yu2016modeling}, UNC+~\cite{yu2016modeling}, G-Ref~\cite{mao2016generation} and ReferIt~\cite{kazemzadeh2014referitgame}.

The UNC dataset contains 19,994 images with 142,209 referring expressions for 50,000 objects. All images and expressions are collected from the MS COCO~\cite{lin2014microsoft} dataset interactively with a two-player game~\cite{kazemzadeh2014referitgame}. Two or more objects of the same object category appear in each image. 

The UNC+ dataset is similar to the UNC dataset. but with a restriction that no location words are allowed in the referring expression. In this case, expressions regarding referred objects totally depend on the appearance and the scene context. It consists of 141,564 expressions for 49,856 objects in 19,992 images.


The G-Ref dataset is also selected from MS COCO. It contains 104,560 expressions referring to 54,822 objects from 26,711 images. Annotations of this dataset come from Amazon Mechanical Turk instead of a two-player game. The average length of expressions is 8.4 words which is longer than that of other datasets (less than 4 words). %It is more challenging to understand referring expressions for segmentation.

The ReferIt dataset is built upon the IAPR TC-12~\cite{escalante2010segmented} dataset. It has 130,525 expressions referring to 96,654 distinct object masks in 19,894 natural images. In addition to objects, it also contains annotations for stuff classes such as water, sky and ground.

\noindent{\bf Evaluation metrics:} Following previous work~\cite{liu2017recurrent, li2018referring, shi2018key}, we use intersection-over-union $(IoU)$ and $prec@X$ as the evaluation metrics. The $IoU$ metric is a ratio between intersection and union of predicted segmentation mask and the ground truth. The $prec@X$ metric measures the percentage of test images with an IoU score higher than the threshold $X$, where $X \in\{ 0.5, 0.6,0.7,0.8,0.9\}$ in the experiments.  


\input fig_seg.tex
\subsection{Experimental Evaluation}\label{sec:result}
%particular for more strict threshold
\noindent{\bf Quantitative results:} Table~\ref{tab:miou} presents comparisons of our method with existing state-of-the-art approaches. Our proposed method consistently outperforms all other methods  on all four datasets. The improvement is particularly significant on the more challenging datasets, such as UNC+ which has no location words and G-Ref which contains longer and richer query expressions. This demonstrates the advantage of capturing long-range dependencies for cross-modal features and understanding the referred objects based on expressions by our model. %The performance gap in test set of ReferIt is relatively small. Probably because the expressions in this dataset are shorter and more concise, which benefits less from the explored cross-modal correlation at dual contexts for this set.


\noindent{\bf Qualitative results:} Figure~\ref{fig:seg} shows some qualitative examples generated by our network. To better understand the benefit of multi-level self-attentive features, we visualize the linguistic representation to show attention distributions at different levels. For a given level, we get the collection of the attention scores $\{a_{p,n,p',n'}: \forall p, \forall n, \forall p', \forall n'\}$ in Eq.~\ref{eq:self2} and average over the dimensions $p$, $p'$ and $n'$. Thereby we can get a vector of length $N$. We repeat this operation for all three levels and finally obtain a matrix of $3\times N$. This matrix is shown in Fig.~\ref{fig:seg} (2nd column). We can see that the attention distribution over words corresponding to a particular feature level is different. Specifically, visual features at different levels tend to pay different attentions on different words, which helps complement detailed visual cues for segmentation masks. The low-level features can concentrate on location words to localize the exact objects in the first and second examples. 
It also completes the linguistic comprehension of the query expression in the bottom three examples by appearance descriptions ( ``small", ``blue" ) and relationship (``second"), and provides fine visual cues to precisely obtain segmentation masks.

\input fig_word.tex

\subsection{Ablation Study}\label{sec:ab}
We perform additional ablation experiments on the UNC dataset to further investigate the relative contribution of each component of our proposed model.

\noindent{\bf Cross-modal self-attentive feature}: This experiment evaluates the effectiveness of the cross-modal self-attentive feature. Similar to the baselines, i.e. multimodal LSTM interaction in~\cite{liu2017recurrent} and convolution integration in~\cite{li2018referring}, we directly take the output of the $Res5$ of the network to test the performance of multimodal feature representation without the multi-level fusion. We use CMSA-W to denote the proposed method in Sec.~\ref{sec:msa}. In addition, we also use a variant of CMSA-S which also uses the same cross-modal self-attentive feature but instead encodes the whole sentence to one single language vector by LSTM. 

As shown in Table~\ref{tab:ab} (top 4 rows), the proposed cross-modal self-attentive feature based approaches achieve significantly better performance than other baselines. Moreover, the word based method CMSA-W outperforms sentence based method CMSA-S which demonstrates the language-to-vision correlation can be better learned together within our  cross-modal self-attention method.% that decouples dependency on encoding visual and language data ahead of integration.

\noindent{\bf Multi-level feature fusion}: This experiment verifies the relative contribution of the proposed gated multi-level fusion. Here we use our cross-modal self-attentive features as inputs and compare several well-known feature fusion techniques, such as Deconv~\cite{noh2015learning} and PPM~\cite{zhao2017pyramid} in semantic segmentation and ConvLSTM~\cite{li2018referring} in referring image segmentation. 

In order to clearly understand the benefit of multi-level gate fusion method, we also develop another self-gated method that uses the same gate generation method in Sec.~\ref{sec:gf} to generate forget gates and directly multiply by its own features without interactions with features from other levels. As presented in the bottom 5 rows in Table~\ref{tab:ab}, the proposed gated multi-level fusion outperforms these other multi-level feature fusion methods.% which demonstrates the multi-level gate integration module also benefits segmentation performance in terms of multi-level feature integration.





\subsection{Visualization}\label{sec:vis}

In this section, we analyse the visualizations of spatial feature representations fed with various query expressions in a given image. The aim of this analysis is to get further insights on the learning of the proposed model. 

We adopt the same technique in~\cite{li2018referring} to generate visual representation maps over spatial locations. We create the visualization by normalizing the strongest activation of the last feature map, which is upsampled to match with the size of original input image. We show the generated heatmaps in Fig.~\ref{fig:word}. 


It can be observed that our model is able to correctly respond to different query expressions with various categories, locations and relationships. For instance, in the second row, when the query is ``woman'' and ``umbrella'', our model highlights every woman and umbrella in the image. Similarly, when the query is ``red'', it captures both the red clothes and the red part of the umbrella. For a more specific phrase such as ``a woman in a green coat'', the model accurately identifies the woman being referred to. 


























